Adaptable Continuous Variable Quantum Network with Finite Size Security

In recent years, continuous-variable quantum key distribution (CV-QKD) has become a promising paradigm for enabling secure communication among multiple end users sharing the same telecommunication backbone. CV-QKD with reverse reconciliation naturally enables scalability from conventional point-to-point links to quantum access networks based on passive quantum broadcasting channels. Here, we report an experimental demonstration on an active $1:4$ multi-user CV quantum network (QN) in the finite-size regime. With $1.25\cdot10^9$ coherent states exchanged on each $11\text{km}$ quantum channel, the highest performance for secret key generation totaling $1.9\cdot10^{-1}$ bits/channel use. Furthermore, we investigate adaptable CV-QN protocols that comprehensively allow network operation in various security and key rates requirements of individual users. The results establish the practical security of CV-QN compatible with existing telecommunication for broad deployment, and allowing additional degree of freedom for connected end users in existing infrastructures.

==> ExperimentalRealization.tex <==
\section{A CV quantum network implementation}
% \subsection{A Network Overview of the Experimental Setup}
% % network topology, node - function and link
% The quantum correlations are established between Alice and four end users, $\text{Bob}_l$, $l \in \{1,2,3,4\}$ with a broadcast topology. The network comprises two types of nodes, active nodes and passive nodes. The active node either prepares and transmits the physical signal carrying the information or detects the received signal to retrieve information. The passive node distributes the signal between the active nodes. In this network shown in Fig.~\ref{fig: the networked system}(a), active nodes include Alice and four Bobs and passive node is the 1:4 optical beam splitter. In the experiment, Alice is connected to each Bob through quantum channels. Alice feeds to the splitter with a single link of $10$km from which individual links of $1$km connect to each Bob. There is no physical link established between the end users. %cannot communicate between themselves.

% % physical equipments of each active node - transmitter and receiver 
% The quantum network with $5$ active interconnected parties, $1$ transmitter and $4$ receivers, constituted a distributed system where clock synchronization was essential. All digital-to-analog converter (DAC) and and analog-to-digital converters (ADCs) were synchronized with one reference clock with $10$ MHz. In addition, a classical channel is established and authenticated between the transmitter and each receiver.

%An overview of the components Fig.~\ref{fig: the networked system}:


% \subsection{Information encoding and distribution}
% In the experimental demonstration of the protocol, we set up one transmitter as Alice and four balanced heterodyne detectors as four Bobs.

\begin{figure*}
    \centering
    %\includegraphics[width=9cm]{1-to-4 experimental schematic.pdf}
    \includegraphics[width=0.95\textwidth]{figure/QPON-1-4-2.pdf}
    \caption{ A continuous variable quantum access network in action in the lab. (a) State preparation station comprises a signal laser, a digital-to-analog converter (DAC), an IQ modulator stabilized by an automatic bias controller (ABC), as well as a variable optical attenuator (VOA) and an isolator. (b) State distribution is assisted with a $1:4$ splitter which splits the coherent states, forming a quantum broadcasting channel that connects N users while distributing quantum correlations evenly among them. The link consists of two segment, a 10 km fiber spool before the $1:4$ splitter represent the communication backbone and at each output of the splitter represent last-mile connection to the end-users. The quantum state sent by Alice is mixed with different quantum noises, consequently. (c) A receiver station comprises a balanced detector (BD) that receives both the signal and the local oscillator (LO) at the 50:50 beamsplitter (BS), while each resultant signal is detected by a photodetector. The analog readout is converted to digital by the analog-to-digital converter (ADC).}
    \label{fig: the networked system}
\end{figure*}

The proof-of-concept continuous-variable quantum network is shown in Fig.~\ref{fig: the networked system}. The system, supporting four active end users, consists of an optical and a digital module, both optimized to ensure finite-size security. In the optical module, the LO was tuned to maintain sufficient clearance above electronic noise without inducing detector instability. In the digital domain, the detector gain was calibrated relative to the LO power. The coupled dynamic variables were optimized together. Additionally, the pilot tone power was adjusted to provide robust phase recovery without saturating the detectors. Since the setup involves four receiver systems, these optimizations were executed iteratively and systematically until the high stability and low noise required were achieved to generate finite-size keys for all four users. To establish quantum correlations, Alice distributed coherent states among the Bobs, encoding information using symbols sampled from a Gaussian distribution. Each symbol's quadrature components, $x_i$ and $p_i$, were independent and identically distributed (i.i.d.) random variables generated by a quantum random number generator (QRNG). Symbols were transmitted at a rate of 125 MBaud and upsampled to 8 samples per symbol using a root-raised cosine (RRC) pulse filter with a roll-off factor of 0.2. Adopting single-sideband modulation, the quantum signal was frequency-shifted by $150$ MHz relative to the carrier and a pilot tone at 10 MHz was frequency-multiplexed to assist the digital signal processing (DSP) process. A 1 GSample/s 16 bits resolution converted the digital samples to an electrical analog signal to drive the two arms of an IQ modulator. Around $1.25\cdot10^9$ symbols were exchanged between Alice and each Bob. The power of the optical signal was controlled by a programmable electrical VOA and sent through a $10$km single-mode fiber channel. Subsequently, the signal was split into four by a passive 1:4 beamsplitter, followed by an additional 1 km fiber channel before entering Bob's receiver stations. Each Bob received the symbols through a distinctive channel corrupted by noise from the channel assumed to be controlled by Eve.

% \newline


% Independent and identically distributed (i.i.d.) random numbers drawn from a quantum random number generator (QRNG) are encoded in both quadrature of the optical field.

%Those quantum symbols were represented by coherent states displaced from the vacuum states to the coordinate of $(q_i, p_i)$ in the phase space. The power was drawn from the signal laser as the displacement was carried out by namely the IQ modulator. \newline

% \newline


% \subsection{Information decoding}
Each Bob detected the signal coming from the channel using radio-frequency (RF) heterodyne detection with a locally generated local oscillator (LLO) at frequency $f_{LO}$ interfering with the signal with the carrier $f_s$ on a 50:50 beamsplitter resulting in a beating frequency $f_b = \abs{f_{LO} - f_s}$ within the electronic detection bandwidth. Each user had a polarization controller to match the polarization of the incoming signal with that of the LLO to maximize the visibility. The signal were detected using balanced detector (BDs) and sampled by a digital-to-analog converter with the sampling rate of $1$Gsample/s. 
% In the phase space, the resultant 

DSP was performed on the received signal to recover the quantum symbols~\cite{chinMachine2021,hajomerLongdistance2024}. A whitening filter was applied to remove time-dependent correlations from the detector’s transfer function. Utilizing the strong pilot signal, we recover the carrier frequency and phase using a machine learning-based technique~\cite{chinMachine2021}. Subsequently, the propagation delay was compensated for, and the signal was downsampled using a matched filter.




==> Theory.tex <==
% updated by Akash
\section{Finite-Size Security Analysis}
%\section{Advanced CV Quantum Network Protocols and Finite-Size Security Analysis}
\label{sec:finite_size_security}
In the asymptotic regime, a basic protocol can generate secret keys when the mutual information of the legitimate parties exceeds the eavesdropper's information-theoretic upper bound. In this section, we analyze the advanced protocols implemented with this CV quantum network in the finite size regime. 

We evaluate the security of the networked system under the Gaussian framework, where the Holevo bound is derived from the symplectic eigenvalues of the system's covariance matrix. In our model, excess noise is treated as an effective contribution at the channel output. To provide a comprehensive security characterization, we analyze three distinct trust models, each defined by the presumed role of the auxiliary users $B_{j \neq k}$.


\subsection{Trust Models and Covariance Formulations}
Let $A$ denote Alice and $\{B_m\}_{m=1}^M$ denote the set of users. For a specific user $B_k$ generating a key with Alice, the Holevo information $\chi_{B_k E}$ is evaluated based on the following state representations:

\begin{itemize}
    \item \textbf{Trusted Users:} All users are considered honest and excluded from Eve's control. The Holevo bound is derived from the global covariance matrix $\Gamma_{A B_1 \cdots B_M}$.
    \item \textbf{Untrusted Users:} All users $B_{j \neq k}$ are treated as potential adversaries. We consider the reduced bipartite covariance matrix $\Gamma_{A B_k}$, effectively tracing out all other users and attributing any inter-user correlations to Eve.
    \item \textbf{Collaborative Disclosure:} Users $B_{j \neq k}$ disclose their measurement outcomes $\bm{y}_{\neg k}$, which Alice and $B_k$ use to condition their shared state. The security analysis employs the conditional covariance matrix $\Gamma_{A B_k \mid \bm{y}_{\neg k}}$.
\end{itemize}

The trusted electronic noise is purified via additional ancillary modes rather than being attributed to the eavesdropper.
\subsection{Finite-Size Key Rate Calculation}
Following the standard treatment for continuous-variable (CV) QKD \cite{Leverrier2010PRA}, we incorporate finite-size effects by performing a worst-case evaluation of the Holevo bound. We assume that error correction precedes parameter estimation, allowing for a block utilization efficiency of $n/N = 1$ \cite{Lupo2018PRL}. The secret key rate $K_k^{\mathrm{FS}}$ (bits per pulse) for user $B_k$ is given by:
\begin{equation}
    K_k^{\mathrm{FS}} = \beta I_{AB_k} - \chi_{B_kE}^{\varepsilon_{\mathrm{PE}}} - \Delta_{\mathrm{tot}}(n),
\end{equation}
where $\beta$ is the reconciliation efficiency and $\chi_{B_kE}^{\varepsilon_{\mathrm{PE}}}$ is the Holevo information maximized over a confidence region with failure probability $\varepsilon_{\mathrm{PE}} = 10^{-10}$. The correction term $\Delta_{\mathrm{tot}}(n)$ accounts for the smoothing of the min-entropy and the failure probability of privacy amplification:
\begin{equation}
    \Delta_{\mathrm{tot}}(n) := (2d+3)\sqrt{\frac{\log_2(2/\bar{\varepsilon})}{n}} + \frac{2}{n}\log_2\left(\frac{1}{\varepsilon_{\mathrm{PA}}}\right),
\end{equation}
where $d$ is the effective Hilbert space dimension, $\bar{\varepsilon}$ is the smoothing parameter, and $\varepsilon_{\mathrm{PA}}$ is the privacy amplification failure probability. The experimental key rates obtained under these conditions are summarized in Table~\ref{tab:finite_size_keyrates_models}.

\begin{table}[ht]
\centering
\caption{Finite-size secret key rates ($K_i$ in bits/channel use) for different trust models and block sizes $N$.}
\label{tab:finite_size_keyrates_models}
\begin{tabular}{c c c c c}
\toprule
$N$ & User & $K_i^{\mathrm{(untrusted)}}$ & $K_i^{\mathrm{(collaborative)}}$ & $K_i^{\mathrm{(trusted)}}$ \\
\midrule
$ 1.25\times10^{9}$ & 1 & 0.0783639 &  0.0986406 & 0.111138 \\
$ 1.25\times10^{9}$ & 2 & 0.0774364 & 0.0968944 &  0.108920 \\
$ 1.25\times10^{9}$ & 3 & 0.0625202 & 0.081329 &  0.0927128 \\
$ 1.25\times10^{9}$ & 4 & 0.0495922 & 0.0666837 &  0.0773247 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Symplectic Evaluation of the Holevo Bound}
For each trust model, we bound Eve's information by assuming a Gaussian collective attack, which is optimal for fixed second moments \cite{GarciaPatron2006}. For a bipartite state $\rho_{AB}$, the Holevo quantity is $ \chi_{BE} = S(\rho_{AB}) - S(\rho_{A|y})$, where $S(\cdot)$ is the von Neumann entropy. These entropies are computed as:
\begin{equation}
    S(\rho) = \sum_j g\left(\frac{\nu_j - 1}{2}\right), \quad g(x) = (x+1)\log_2(x+1) - x\log_2 x,
\end{equation}
where $\{\nu_j\}$ are the symplectic eigenvalues of the relevant covariance matrix (global, reduced, or conditional) and $\{\tilde{\nu}_j\}$ are the eigenvalues of the state after Bob’s measurement. In the collaborative model, the mutual information is similarly computed using the conditioned data:
\begin{equation}
    I_{A B_k}^{\mathrm{collab}} \equiv I(A:B_k \mid \bm{y}_{\neg k}).
\end{equation}


==> Theory2.tex <==
\section{Finite-size Continuous Variable Network Protocol and Security Analysis}
\label{sec:finite_size_security}
% covariance matrix for all three protocols 
We work within the Gaussian framework, for which the security analysis under collective attacks is fully determined by the covariance matrix of the joint state shared by Alice and all users. In this sense, the covariance matrix of the global network state is the fundamental object from which all relevant security quantities are obtained. Throughout this section, we operate strictly in the finite-size regime: all covariance matrices are constructed from the worst-case parameter values compatible with the parameter-estimation confidence region described in Sec.~\ref{sec:PE}, with failure probability \(\epsilon_{\rm PE}=10^{-10}\). In particular, rather than using the maximum-likelihood estimates of the channel transmittance and excess noise, we substitute the least favorable values within the confidence region, namely those that minimize the secret key rate. This convention applies uniformly to all covariance matrices appearing in this section, whether reduced, global, or conditional. The distinction between the different protocol scenarios considered below lies only in how this worst-case global covariance matrix is used, namely whether one evaluates reduced, global, or conditional covariance matrices according to the operational role assigned to the non-target users.

Let $A$ denote Alice and $\{B_m\}_{m=1}^{M}$ the set of users. When Alice establishes a key with a specific user $B_k$, the finite-size secret key rate is given by
\begin{equation}
    K_k^{\mathrm{FS}}
    =
    \beta I_{AB_k}
    -
    \chi_{B_kE}^{\varepsilon_{\mathrm{PE}}}
    -
    \Delta(N),
\end{equation}
where $\beta$ is the reconciliation efficiency, $I_{AB_k}$ is the classical mutual information between Alice and $B_k$, and $\chi_{B_kE}^{\varepsilon_{\mathrm{PE}}}$ is the Holevo information evaluated for the worst-case covariance matrix within the confidence region associated with the parameter-estimation failure probability $\varepsilon_{\mathrm{PE}}=10^{-10}$. The term $\Delta(N)$ accounts for the finite-size composable correction.

Following the standard finite-size treatment of CV-QKD \cite{Leverrier2010PRA}, the finite-size correction is dominated by the smooth-min-entropy contribution. Since in our protocol the raw key is binary, we take the effective Hilbert-space dimension to be $2$, which gives the prefactor $2\times2+3=7$. Furthermore, for the block sizes considered here, the privacy-amplification contribution is negligible compared with the square-root term. Assuming error correction before parameter estimation so that $n/N=1$ \cite{Lupo2018PRL}, we therefore use
\begin{equation}
    \Delta(N)
    =
    7\sqrt{\frac{\log_2(2\times 10^{10})}{N}},
\end{equation}
where $N$ is the number of exchanged pulses contributing to the raw key.
For Gaussian states, the Holevo quantity is obtained from the symplectic eigenvalues of the relevant covariance matrix through the von Neumann entropy
\begin{equation}
    S(\rho)=\sum_j g\!\left(\frac{\nu_j-1}{2}\right),
    \qquad
    g(x)=(x+1)\log_2(x+1)-x\log_2x.
\end{equation}
Thus, once the covariance matrix appropriate to a given scenario is specified, the corresponding mutual-information and Holevo terms are fixed.

We consider three distinct scenarios. In the trusted case, only one user $B_k$ generates a key with Alice, while all remaining users are assumed trusted and do not participate in the key-generation step. The mutual information is therefore evaluated from the reduced covariance matrix $\Gamma_{AB_k}$, since it only concerns Alice and the target user. However, the Holevo bound is evaluated from the global covariance matrix $\Gamma_{AB_1\cdots B_M}$, because the remaining users are excluded from Eve's system. This gives an optimistic single-user key rate for the selected user.

In the collaborative case, again only one user $B_k$ generates a key with Alice, but the remaining users assist by publicly disclosing their measurement outcomes. The detector noise associated with these assisting users is not assumed trusted. The relevant state is then the conditional state of Alice and $B_k$ given the disclosed outcomes of the other users. Accordingly, both the mutual information and the Holevo information are evaluated from the conditional covariance matrix
\begin{equation}
    \Gamma_{AB_k \mid \bm{y}_{\neg k}},
\end{equation}
where $\bm{y}_{\neg k}$ denotes the collection of measurement outcomes disclosed by all users other than $B_k$. In this scenario the mutual information is correspondingly conditioned on the disclosed data,
\begin{equation}
    I_{AB_k}^{\mathrm{collab}}
    \equiv
    I(A:B_k \mid \bm{y}_{\neg k}).
\end{equation}

In the untrusted case, all non-target users are treated as untrusted and effectively assigned to the eavesdropper. As a result, each user can be analysed independently, since no benefit is obtained from the remaining users. For a given user $B_k$, both the mutual information and the Holevo bound are evaluated from the reduced covariance matrix $\Gamma_{AB_k}$. Operationally, this attributes all correlations involving the other users to Eve.

The finite-size key rates obtained for these three scenarios are summarized in Table~\ref{tab:finite_size_keyrates_models}. The trusted and collaborative cases should both be understood as single-user key-generation settings with different assumptions on the role of the remaining users, whereas the untrusted case naturally leads to independent user-wise key-rate evaluation.

\begin{table}[ht]
\centering
\caption{Finite-size secret key rates ($K_i$ in bits/channel use) for different trust models and block sizes $N$.}
\label{tab:finite_size_keyrates_models}
\begin{tabular}{c c c c c}
\toprule
$N$ & User & $K_i^{\mathrm{(untrusted)}}$ & $K_i^{\mathrm{(collaborative)}}$ & $K_i^{\mathrm{(trusted)}}$ \\
\midrule
$ 1.25\times10^{9}$ & 1 & 0.0783639 &  0.0976479 & 0.11056513 \\
$ 1.25\times10^{9}$ & 2 & 0.0774364 & 0.0959016 &  0.10834679 \\
$ 1.25\times10^{9}$ & 3 & 0.0625202 & 0.0803363 &  0.09213961 \\
$ 1.25\times10^{9}$ & 4 & 0.0495922 & 0.0656909 &  0.07633193 \\
\bottomrule
\end{tabular}
\end{table}

To characterize the optimal total key that the users can establish with Alice, it is not sufficient to sum the individually evaluated trusted-user rates. Those rates are obtained by selecting one user at a time as the key-generating user, while treating all remaining users as trusted side systems. Repeating this optimistic single-user evaluation for several users reuses shared correlations, and therefore the sum of the trusted per-user rates can exceed the total key content actually available in the collective user system. For this reason, the trusted-user rates reported above should be interpreted as single-user benchmark rates rather than as parallel simultaneously achievable key rates.

The appropriate quantity for the total key available across all users is instead obtained by considering all Bobs collectively, as introduced in our earlier multi-user analysis \cite{vsqj-ndkn}. Denoting the full user system by $\bm{B}:=(B_1,\dots,B_M)$, the corresponding collective key rate is
\begin{equation}
    K(A:\bm{B})
    =
    I(A:\bm{B})
    -
    \chi_{\bm{B}E},
\end{equation}
where
\begin{equation}
    \chi_{\bm{B}E}
    =
    S(\rho_{A\bm{B}})
    -
    S(\rho_{A\mid \bm{B}}).
\end{equation}
This collective quantity bounds the total key content available in the joint measurement data of all users.

The collective rate can then be decomposed into individual user contributions by successive conditioning. Using the chain rule for mutual information,
\begin{equation}
    I(A:B_1,\dots,B_M)
    =
    \sum_{k=1}^{M}
    I\!\left(A:B_k \mid B_1,\dots,B_{k-1}\right),
\end{equation}
while the Holevo contribution admits the telescopic decomposition
\begin{equation}
\begin{split}
    &S(\rho_{AB_1\cdots B_M}) - S(\rho_{A\mid B_1\cdots B_M}) \\
    &=
    \sum_{k=1}^{M}
    \left[
    S(\rho_{A\mid B_1\cdots B_{k-1}})
    -
    S(\rho_{A\mid B_1\cdots B_k})
    \right].
\end{split}
\end{equation}
Combining these expressions yields
\begin{equation}
    K(A:B_1,\dots,B_M)
    =
    \sum_{k=1}^{M} K_k^{\mathrm{dec}},
\end{equation}
with
\begin{equation}
\begin{split}
    K_k^{\mathrm{dec}}
    &:=
    I\!\left(A:B_k \mid B_1,\dots,B_{k-1}\right) \\
    &\quad
    -
    \left[
    S(\rho_{A\mid B_1\cdots B_{k-1}})
    -
    S(\rho_{A\mid B_1\cdots B_k})
    \right].
\end{split}
\end{equation}

\begin{table*}[ht]
\centering
\caption{Decomposition of the collective key rate into individual user contributions for all user orders. Each row corresponds to a different conditioning order used in the chain-rule decomposition of the collective key rate \(K(A:B_1,\dots,B_4)\). The entries \(K_1,K_2,K_3,K_4\) denote the individual user contributions obtained under that decomposition. While the allocation of key among users depends on the chosen order, the total sum \(\sum_{i=1}^4 K_i\) is invariant and equals the collective key rate, \(0.38205215\) bits per channel use, for all orders.}
\label{tab:all_key_orders}
\begin{tabular}{c c c c c}
\toprule
Order & $K_1$ & $K_2$ & $K_3$ & $K_4$ \\
\midrule
$(B_1,B_2,B_3,B_4)$ & 0.11056513 & 0.10712770 & 0.09016792 & 0.07419140 \\
$(B_1,B_2,B_4,B_3)$ & 0.11056513 & 0.10712770 & 0.07459115 & 0.08976817 \\
$(B_1,B_3,B_2,B_4)$ & 0.11056513 & 0.09102361 & 0.10627201 & 0.07419140 \\
$(B_1,B_3,B_4,B_2)$ & 0.11056513 & 0.09102361 & 0.07465306 & 0.10581035 \\
$(B_1,B_4,B_2,B_3)$ & 0.11056513 & 0.07535383 & 0.10636503 & 0.08976817 \\
$(B_1,B_4,B_3,B_2)$ & 0.11056513 & 0.07535383 & 0.09032284 & 0.10581035 \\
$(B_2,B_1,B_3,B_4)$ & 0.10834679 & 0.10934604 & 0.09016792 & 0.07419140 \\
$(B_2,B_1,B_4,B_3)$ & 0.10834679 & 0.10934604 & 0.07459115 & 0.08976817 \\
$(B_2,B_3,B_1,B_4)$ & 0.10834679 & 0.09106191 & 0.10845204 & 0.07419140 \\
$(B_2,B_3,B_4,B_1)$ & 0.10834679 & 0.09106191 & 0.07467404 & 0.10796940 \\
$(B_2,B_4,B_1,B_3)$ & 0.10834679 & 0.07538783 & 0.10854935 & 0.08976817 \\
$(B_2,B_4,B_3,B_1)$ & 0.10834679 & 0.07538783 & 0.09034812 & 0.10796940 \\
$(B_3,B_1,B_2,B_4)$ & 0.09213961 & 0.10944913 & 0.10627201 & 0.07419140 \\
$(B_3,B_1,B_4,B_2)$ & 0.09213961 & 0.10944913 & 0.07465306 & 0.10581035 \\
$(B_3,B_2,B_1,B_4)$ & 0.09213961 & 0.10726909 & 0.10845204 & 0.07419140 \\
$(B_3,B_2,B_4,B_1)$ & 0.09213961 & 0.10726909 & 0.07467404 & 0.10796940 \\
$(B_3,B_4,B_1,B_2)$ & 0.09213961 & 0.07546865 & 0.10863354 & 0.10581035 \\
$(B_3,B_4,B_2,B_1)$ & 0.09213961 & 0.07546865 & 0.10647449 & 0.10796940 \\
$(B_4,B_1,B_2,B_3)$ & 0.07633193 & 0.10958702 & 0.10636503 & 0.08976817 \\
$(B_4,B_1,B_3,B_2)$ & 0.07633193 & 0.10958702 & 0.09032284 & 0.10581035 \\
$(B_4,B_2,B_1,B_3)$ & 0.07633193 & 0.10740269 & 0.10854935 & 0.08976817 \\
$(B_4,B_2,B_3,B_1)$ & 0.07633193 & 0.10740269 & 0.09034812 & 0.10796940 \\
$(B_4,B_3,B_1,B_2)$ & 0.07633193 & 0.09127633 & 0.10863354 & 0.10581035 \\
$(B_4,B_3,B_2,B_1)$ & 0.07633193 & 0.09127633 & 0.10647449 & 0.10796940 \\
\bottomrule
\end{tabular}
\end{table*}
Therefore, the collective key rate is not the sum of the independently evaluated trusted-user rates, but the sum of individual contributions defined through successive conditioning. This decomposition ensures that correlations shared among different users are accounted for only once.

This interpretation is not primarily about the temporal ordering of reconciliation. In practice, all users may transmit reconciliation information to Alice, and Alice may reconstruct the relevant measurement data for all of them. The point is instead that, once the collective information is available, the attribution of the total key content to individual users must be performed through conditional decomposition in order to remove correlations among users and avoid double counting. Different conditioning orders generally lead to different individual user contributions, while the collective sum rate remains unchanged. Hence, the total key content of the network is fixed by the joint state, whereas its distribution among users depends on how the collective rate is decomposed.

==> draft.tex <==
%Secure communication necessitates a new communication protocol and implementation against potential malicious will to intercept and decode the communicated information, equipped with ever-growing computation capacity. It is desirable to have such technology coexist with current telecommunication in metropolitan networks for attainable deployment and commercialization.  

 %In recent years, continuous-variable (CV) quantum communication has become a promising paradigm with its natural scalability for enabling secure communication among multiple end users sharing the same telecommunication backbone. 
 %Modern cryptography safeguarding communications sharing public infrastructure is under risk due to the promise of quantum computing.

 %Those equipped with the accelerating growth of computation capacity from both the classical and quantum world will try to intercept and decode the critical communicated information ~\cite{cain2026shor}. 
